Circumstellar interaction models for the early bolometric light curve of SN 2023ixf

SNe II show growing evidence of interaction with CSM surrounding their progenitor stars as a consequence of enhanced mass loss during the last years of the progenitor's life. We present an analysis of the progenitor mass-loss history of SN2023ixf, a nearby SN II showing signs of interaction. We calculate the early-time bolometric light curve (LC) for SN2023ixf based on the integration of the observed flux covering UV, optical and NIR bands, and black-body extrapolations for the unobserved flux. Our calculations spot the sudden increase to maximum luminosity and temperature, in addition to the subsequent fall, displaying an evident peak. This is the first time that this phase can be precisely estimated for a SN II showing interesting characteristics as: 1) slope changes during the rise to maximum luminosity; and 2) a very sharp peak with a maximum luminosity of $\sim$3$\times$10$^{45}$erg s$^{-1}$. We use the bolometric LC of SN2023ixf to test the calibrations of bolometric corrections against colours from the literature. In addition, we include SN2023ixf into some of the available calibrations to extend their use to earlier epochs. Comparison of the observed bolometric LC to SN II explosion models with CSM interaction suggests a progenitor mass-loss rate of 3$\times$10$^{-3}M_{\odot}$yr$^{-1}$ confined to 12000$R_{\odot}$ and a wind acceleration parameter of $\beta$=5. This model reproduces the early bolometric LC, expansion velocities, and the epoch of disappearance of interacting lines in the spectra. This model indicates that the wind was launched $\sim$80yr before the explosion. If the effect of the wind acceleration is not taken into account, the enhanced wind must have developed over the final months to years prior to the SN, which may not be consistent with the lack of outburst detection in pre-explosion images over the last $\sim$20yr before explosion.

==> tables/luminosity.tex <==
\longtab[1]{
\begin{longtable}{ccc}
\caption{Bolometric luminosities for SN~2023ixf.}
\label{table:luminosity}
\\ \hline\hline\noalign{\smallskip}
MJD & Luminosity [erg s$^{-1}$] & Error [erg s$^{-1}$] \\
\hline\noalign{\smallskip}
\endfirsthead
\caption{continued.}\\
\hline\hline\noalign{\smallskip}
MJD & Luminosity [erg] & Error [erg] \\
\hline\noalign{\smallskip}
\endhead
\hline\noalign{\smallskip}
\endfoot
%%
60084.6500 & 6.20e+42 & 2.12e+41 \\
60084.9597 & 1.15e+43 & 4.40e+41 \\
60085.0000 & 1.26e+43 & 5.64e+41 \\
60085.0494 & 1.33e+43 & 5.13e+41 \\
60085.1327 & 1.43e+43 & 4.82e+41 \\
60085.2122 & 1.49e+43 & 4.38e+41 \\
60085.3162 & 1.56e+43 & 4.24e+41 \\
60085.5941 & 1.91e+43 & 6.72e+41 \\
60085.6000 & 2.24e+43 & 7.56e+41 \\
60085.6400 & 1.87e+43 & 1.08e+42 \\
60085.6400 & 1.16e+43 & 5.56e+41 \\
60085.8778 & 2.48e+43 & 1.84e+42 \\
60085.8940 & 3.75e+43 & 2.99e+42 \\
60085.9596 & 5.89e+43 & 5.76e+42 \\
60086.0000 & 1.12e+44 & 1.64e+43 \\
60086.0801 & 1.87e+44 & 2.78e+43 \\
60086.2200 & 3.34e+45 & 1.69e+45 \\
60086.2630 & 4.75e+44 & 1.07e+44 \\
60086.4210 & 2.07e+44 & 2.84e+43 \\
60086.6000 & 9.99e+43 & 1.01e+43 \\
60086.6300 & 5.09e+43 & 3.09e+42 \\
60086.8788 & 3.24e+43 & 1.65e+42 \\
60086.8990 & 5.97e+43 & 1.26e+42 \\
60086.9000 & 3.46e+43 & 1.88e+42 \\
60087.0831 & 3.69e+43 & 2.33e+42 \\
60087.1860 & 3.27e+43 & 1.99e+42 \\
60087.2000 & 3.20e+43 & 1.92e+42 \\
60087.2540 & 2.71e+43 & 1.86e+42 \\
60087.5396 & 2.25e+43 & 1.06e+42 \\
60087.5800 & 3.19e+43 & 1.59e+42 \\
60087.8700 & 2.11e+43 & 1.11e+42 \\
60087.8739 & 1.93e+43 & 8.65e+41 \\
60087.9070 & 1.87e+43 & 8.83e+41 \\
60088.1920 & 1.70e+43 & 7.08e+41 \\
60088.2540 & 1.49e+43 & 6.58e+41 \\
60088.4000 & 1.57e+43 & 5.94e+41 \\
60088.4200 & 1.40e+43 & 4.94e+41 \\
60088.4994 & 1.56e+43 & 6.26e+41 \\
60088.7500 & 1.60e+43 & 7.79e+41 \\
60088.8788 & 1.37e+43 & 5.04e+41 \\
60088.9540 & 1.32e+43 & 4.69e+41 \\
60089.1253 & 1.27e+43 & 4.54e+41 \\
60089.2027 & 1.25e+43 & 4.34e+41 \\
60089.2500 & 1.21e+43 & 4.41e+41 \\
60089.3451 & 1.22e+43 & 4.38e+41 \\
60089.6700 & 1.36e+43 & 4.45e+41 \\
60089.7700 & 1.18e+43 & 4.89e+41 \\
60089.8840 & 1.11e+43 & 3.21e+41 \\
60089.9157 & 1.10e+43 & 3.15e+41 \\
60090.1075 & 1.08e+43 & 2.85e+41 \\
60090.2435 & 1.07e+43 & 2.71e+41 \\
60090.4210 & 9.74e+42 & 2.32e+41 \\
60090.6400 & 1.09e+43 & 3.32e+41 \\
60090.9847 & 1.04e+43 & 2.09e+41 \\
60091.0765 & 1.05e+43 & 2.05e+41 \\
60091.1279 & 1.05e+43 & 2.11e+41 \\
60091.4200 & 1.02e+43 & 2.27e+41 \\
60091.5227 & 1.06e+43 & 2.03e+41 \\
60091.6100 & 1.12e+43 & 2.71e+41 \\
60091.6500 & 9.49e+42 & 1.63e+41 \\
60091.9320 & 9.98e+42 & 1.75e+41 \\
60092.0130 & 9.80e+42 & 1.68e+41 \\
60092.1227 & 9.78e+42 & 1.73e+41 \\
60092.2139 & 9.58e+42 & 1.69e+41 \\
60092.4210 & 9.11e+42 & 2.12e+41 \\
60092.6300 & 9.70e+42 & 1.96e+41 \\
60092.8538 & 9.07e+42 & 1.58e+41 \\
60093.0646 & 8.91e+42 & 1.60e+41 \\
60093.1374 & 8.90e+42 & 1.58e+41 \\
60093.4210 & 8.11e+42 & 1.42e+41 \\
60093.8776 & 8.65e+42 & 1.57e+41 \\
60093.9026 & 8.57e+42 & 1.55e+41 \\
60094.1572 & 8.56e+42 & 1.63e+41 \\
60094.7400 & 8.49e+42 & 1.63e+41 \\
60095.0823 & 8.29e+42 & 1.53e+41 \\
60095.1789 & 8.27e+42 & 1.54e+41 \\
60095.4862 & 8.09e+42 & 1.46e+41 \\
60095.5000 & 8.16e+42 & 8.86e+40 \\
60095.5000 & 7.94e+42 & 9.34e+40 \\
60095.5347 & 7.91e+42 & 8.93e+40 \\
60095.9374 & 7.69e+42 & 6.57e+40 \\
60096.0006 & 7.67e+42 & 6.77e+40 \\
60096.1301 & 7.59e+42 & 6.55e+40 \\
60096.3000 & 7.51e+42 & 6.48e+40 \\
60096.4000 & 7.66e+42 & 8.46e+40 \\
60096.6000 & 6.94e+42 & 6.55e+40 \\
60096.8770 & 7.52e+42 & 1.15e+41 \\
60096.8770 & 7.53e+42 & 1.15e+41 \\
60096.9247 & 6.65e+42 & 1.61e+41 \\
60097.1231 & 6.58e+42 & 1.45e+41 \\
60097.7100 & 6.63e+42 & 1.09e+41 \\
60097.9271 & 6.29e+42 & 1.17e+41 \\
60098.0794 & 6.45e+42 & 1.16e+41 \\
60098.2406 & 6.51e+42 & 1.16e+41 \\
60098.3000 & 6.63e+42 & 1.12e+41 \\
60098.5000 & 6.53e+42 & 9.66e+40 \\
60098.5597 & 7.01e+42 & 1.27e+41 \\
60098.6200 & 6.80e+42 & 1.37e+41 \\
60098.9460 & 6.99e+42 & 1.21e+41 \\
60099.0000 & 7.01e+42 & 1.13e+41 \\
60099.0921 & 7.21e+42 & 1.28e+41 \\
60099.6100 & 6.56e+42 & 9.36e+40 \\
60099.6300 & 6.05e+42 & 1.24e+41 \\
60099.9161 & 6.13e+42 & 8.58e+40 \\
60100.6200 & 5.59e+42 & 1.18e+41 \\
60100.7200 & 5.77e+42 & 2.15e+41 \\
60100.9054 & 5.90e+42 & 8.31e+40 \\
60101.6200 & 5.71e+42 & 1.16e+41 \\
\end{longtable}
}

